Multi-functional Wafer-Scale Van der Waals Heterostructures and Polymorphs

Van der Waals heterostructures have promised the realisation of artificial materials with multiple physical phenomena such as giant optical nonlinearities, spin-to-charge interconversion in spintronics and topological carrier protection, in a single layered device through an infinitely diverse set of quantum materials. However, most efforts have only focused on exfoliated material that inherently limits both the dimensions of the materials and the scalability for applications. Here, we show the epitaxial growth of large area heterostructures of topological insulators (Bi2Se3), transition metal dichalcogenides (TMDs, WSe2) and ferromagnets (Co), resulting in the combination of functionalities including tuneable optical nonlinearities, spin-to-charge conversion and magnetic proximity effects. This is demonstrated through coherent phase resolved terahertz currents, bringing novel functionalities beyond those achievable in simple homostructures. In particular, we show the role of different TMD polymorphs, with the simple change of one atomic monolayer of the artificial material stack entirely changing its optical, electrical and magnetic properties. This epitaxial integration of diverse two-dimensional materials offers foundational steps towards diverse perspectives in quantum material engineering, where the material polymorph can be controlled at technological relevant scales for coupling applications in, for example, van der Waals nonlinear optics, optoelectronics, spintronics, multiferroics and coherent current control.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
